Token Homogenization under Positional Bias

This paper investigates token homogenization - the convergence of token representations toward uniformity across transformer layers and its relationship to positional bias in large language models. We empirically examine whether homogenization occurs and how positional bias amplifies this effect. Through layer-wise similarity analysis and controlled experiments, we demonstrate that tokens systematically lose distinctiveness during processing, particularly when biased toward extremal positions. Our findings confirm both the existence of homogenization and its dependence on positional attention mechanisms.

==> review.tex <==
\newpage

\onecolumn
\section*{Review Instructions}
For each section, identify unclear or confusing elements (e.g., unexplained importance of work in abstract, unsupported hypotheses). Provide recommendations for improvements. Use the template below for structured evaluation.

\hrulefill

\section*{Reviewer One}
\section*{Report Structure}
\begin{description}
    \item[Evaluation Criteria:] Does the report include all required sections: Abstract, Introduction and Related Work, Methods, and (Preliminary) Results?
    \item[Max Points:] 1
    \item[Your Points:] 1
    \item[Comments:] All required sections are presented (except for Work Plan, but if I understand correctly, it is specified in Future Steps).
\end{description}

\section*{Abstract}
\begin{description}
    \item[Evaluation Criteria 1:] Does the abstract clearly state the significance of the work?
    \item[Evaluation Criteria 2:] Does the abstract clearly outline the objectives or key activities of the project?
    \item[Max Points:] 1
    \item[Your Points:] 1
    \item[Comments:] The abstract is there, it reflects the essence, also the description of the practical value can be added.
\end{description}

\section*{Introduction and Related Work}
\textit{Note: Evaluate as two separate sections}
\begin{description}
    \item[Evaluation Criteria 1:] Does the introduction provide a broad overview of the project topic?
    \item[Evaluation Criteria 2:] Does the introduction clearly explain the importance of this specific work?
    \item[Evaluation Criteria 3:] Does the literature review clearly summarize relevant prior work?
    \item[Evaluation Criteria 4:] Does the literature review effectively position this project within existing research, justifying its contribution or novelty?
    \item[Max Points:] 2
    \item[Your Points:] 2
    \item[Comments:] The introduction is comprehensive and clear. As for additions, it would be beneficial to include something like "Our contribution" at the end to more clearly describe the connection to your work. It would also be beneficial to further elaborate on the consequences of homogenisation for downstream tasks.
\end{description}

\section*{Methods}
\begin{description}
    \item[Evaluation Criteria 1:] Does the methods section detail the experimental methodology to be used?
    \item[Evaluation Criteria 2:] Does it outline a complete plan of work sufficient for producing a final paper?
    \item[Evaluation Criteria 3:] Is the proposed methodology and work plan justified by references to previous related work?
    \item[Max Points:] 2
    \item[Your Points:] 1.7
    \item[Comments:] There is a clear description of the methods, spectral metrics, MAUVE, and the protocol with synthetic datasets. What is missing, is a detailed description of the experimental parameters and how the results will ultimately be statistically compared.
\end{description}

\section*{Work Plan}
\textit{Note: May be integrated into other sections if explicitly addressed}
\begin{description}
    \item[Evaluation Criteria 1:] Is the overall plan of work clearly defined?
    \item[Evaluation Criteria 2:] Is the plan realistic given the time frame and resources?
    \item[Evaluation Criteria 3:] If completed as described, is it likely to yield publishable results?
    \item[Max Points:] 2
    \item[Your Points:] 1.5
    \item[Comments:] There is no separate section - the plan is divided between Validation Protocol and Future Steps, but the steps are generally clear. Also the plan is realistic but could benefit from a risk-mitigation strategy, e.g., alternative models if LLaMA-3 experiments fail.
    
\end{description}

\section*{Preliminary Results}
\begin{description}
    \item[Evaluation Criteria 1:] Do the preliminary results demonstrate the viability of the proposed methods?
    \item[Evaluation Criteria 2:] Do the preliminary results justify continuing with the chosen work plan? (i.e., do they suggest the plan is likely to succeed?)
    \item[Max Points:] 2
    \item[Your Points:] 1.8
    \item[Comments:] The results are partially obtained, with visualisations of anisotropy (Fig. 1) and attention heatmaps (Fig. 2–3) showing a decrease in diversity and positional bias at the ends of the sequence for LLaMA. 
    The visualisations require a minor formatting correction, but this is not critical. Further quantitative analysis is expected, and results for other models and metrics also.
\end{description}

\hrulefill

\section*{Reviewer Two}

\section*{Report Structure}
\begin{description}
    \item[Evaluation Criteria:] Does the report include all required sections: Abstract, Introduction and Related Work, Methods, and (Preliminary) Results?
    \item[Max Points:] 1
    \item[Your Points:] 1
    \item[Comments:] All required sections are presented.
\end{description}

\section*{Abstract}
\begin{description}
    \item[Evaluation Criteria 1:] Does the abstract clearly state the significance of the work?
    \item[Evaluation Criteria 2:] Does the abstract clearly outline the objectives or key activities of the project?
    \item[Max Points:] 1
    \item[Your Points:] 0.7
    \item[Comments:] Objectives are clearly outline, however the abstract could more clearly articulate why this research matters.
\end{description}

\section*{Introduction and Related Work}
\textit{Note: Evaluate as two separate sections}
\begin{description}
    \item[Evaluation Criteria 1:] Does the introduction provide a broad overview of the project topic?
    \item[Evaluation Criteria 2:] Does the introduction clearly explain the importance of this specific work?
    \item[Evaluation Criteria 3:] Does the literature review clearly summarize relevant prior work?
    \item[Evaluation Criteria 4:] Does the literature review effectively position this project within existing research, justifying its contribution or novelty?
    \item[Max Points:] 2
    \item[Your Points:] 2
    \item[Comments:] The introduction offers a clear and concise overview. It introduces key concepts - positional bias and token homogenization, and provides background on their importance in transformer-based language models. While the technical focus is clear, the introduction could benefit from one or two sentences offering higher-level motivation, how these phenomena affect practical outcomes in LLMs.

\end{description}

\section*{Methods}
\begin{description}
    \item[Evaluation Criteria 1:] Does the methods section detail the experimental methodology to be used?
    \item[Evaluation Criteria 2:] Does it outline a complete plan of work sufficient for producing a final paper?
    \item[Evaluation Criteria 3:] Is the proposed methodology and work plan justified by references to previous related work?
    \item[Max Points:] 2
    \item[Your Points:] 1.7
    \item[Comments:] The Methods section outlines the metrics used in the study, however, it lacks a detailed description of the overall methodology. The planned work is clearly completed and supported by appropriate references to related research.
\end{description}

\section*{Work Plan}
\textit{Note: May be integrated into other sections if explicitly addressed}
\begin{description}
    \item[Evaluation Criteria 1:] Is the overall plan of work clearly defined?
    \item[Evaluation Criteria 2:] Is the plan realistic given the time frame and resources?
    \item[Evaluation Criteria 3:] If completed as described, is it likely to yield publishable results?
    \item[Max Points:] 2
    \item[Your Points:] 2
    \item[Comments:] The plan is partially well-defined. The major steps—visualizing additional metrics, analyzing synthetic datasets, and comparing positional configurations are outlined.
\end{description}

\section*{Preliminary Results}
\begin{description}
    \item[Evaluation Criteria 1:] Do the preliminary results demonstrate the viability of the proposed methods?
    \item[Evaluation Criteria 2:] Do the preliminary results justify continuing with the chosen work plan? (i.e., do they suggest the plan is likely to succeed?)
    \item[Max Points:] 2
    \item[Your Points:] 2
    \item[Comments:] The preliminary results demonstrate the viability of the proposed methods. Initial layer-wise analysis confirms the presence of token homogenization and its amplification by positional bias, aligning well with the study’s hypotheses. These findings validate the chosen metrics and justify further investigation through the planned synthetic dataset experiments.
\end{description}


\hrulefill

\section*{Reviewer Three}

\section*{Report Structure}
\begin{description}
    \item[Evaluation Criteria:] Does the report include all required sections: Abstract, Introduction and Related Work, Methods, and (Preliminary) Results?
    \item[Max Points:] 1
    \item[Your Points:] 
    \item[Comments:] 
\end{description}

\section*{Abstract}
\begin{description}
    \item[Evaluation Criteria 1:] Does the abstract clearly state the significance of the work?
    \item[Evaluation Criteria 2:] Does the abstract clearly outline the objectives or key activities of the project?
    \item[Max Points:] 1
    \item[Your Points:] 
    \item[Comments:]
\end{description}

\section*{Introduction and Related Work}
\textit{Note: Evaluate as two separate sections}
\begin{description}
    \item[Evaluation Criteria 1:] Does the introduction provide a broad overview of the project topic?
    \item[Evaluation Criteria 2:] Does the introduction clearly explain the importance of this specific work?
    \item[Evaluation Criteria 3:] Does the literature review clearly summarize relevant prior work?
    \item[Evaluation Criteria 4:] Does the literature review effectively position this project within existing research, justifying its contribution or novelty?
    \item[Max Points:] 2
    \item[Your Points:] 
    \item[Comments:] 
\end{description}

\section*{Methods}
\begin{description}
    \item[Evaluation Criteria 1:] Does the methods section detail the experimental methodology to be used?
    \item[Evaluation Criteria 2:] Does it outline a complete plan of work sufficient for producing a final paper?
    \item[Evaluation Criteria 3:] Is the proposed methodology and work plan justified by references to previous related work?
    \item[Max Points:] 2
    \item[Your Points:] 
    \item[Comments:] 
\end{description}

\section*{Work Plan}
\textit{Note: May be integrated into other sections if explicitly addressed}
\begin{description}
    \item[Evaluation Criteria 1:] Is the overall plan of work clearly defined?
    \item[Evaluation Criteria 2:] Is the plan realistic given the time frame and resources?
    \item[Evaluation Criteria 3:] If completed as described, is it likely to yield publishable results?
    \item[Max Points:] 2
    \item[Your Points:] 
    \item[Comments:] 
\end{description}

\section*{Preliminary Results}
\begin{description}
    \item[Evaluation Criteria 1:] Do the preliminary results demonstrate the viability of the proposed methods?
    \item[Evaluation Criteria 2:] Do the preliminary results justify continuing with the chosen work plan? (i.e., do they suggest the plan is likely to succeed?)
    \item[Max Points:] 2
    \item[Your Points:]
    \item[Comments:] 
\end{description}


\newpage
\section*{FINAL REVIEW}

\definecolor{rating5}{RGB}{0,115,0}
\definecolor{rating4}{RGB}{0,140,0}
\definecolor{rating3}{RGB}{200,150,0}
\definecolor{rating2}{RGB}{210,80,0}
\definecolor{rating1}{RGB}{180,0,0}

\section*{Publication Policy Note}
\begin{center}
\fbox{\parbox{0.9\textwidth}{%
    \textbf{Important Clarifications:}
    \begin{itemize}
        \item SSPP is a \textbf{non-exclusive publication venue} for summer school proceedings
        \item Submission to SSPP \textit{does not} prevent future publication in ranked venues
        \item SSPP is \textit{not} an indexed journal/conference (Scopus, WoS, etc.)
        \item Publication here \textbf{does not constitute prior publication} for conference/journal submissions
        \item Authors retain full copyright for future submissions
        \item \textit{Note:} Policies may vary at future venues; always verify target venue rules.\\ 
        Non-indexed archival publications typically don't preclude future submissions.
    \end{itemize}
}}
\end{center}
\section*{Goal of SSPP}
Select papers that \textbf{advance research} by:
\begin{enumerate}[label=(\alph*)]
    \item Preliminary investigations of novel directions
    \item Critical analysis of emerging technology applications
    \item Empirical experiments providing foundations for future studies
\end{enumerate}

\\

\noindent The main goal of the review is to help the authors improve their paper and learn something new about doing science. We expect the feedback to be actionable. It can include specific actions such as writing, designing experiments, or the method. For example, you can suggest comparing with an additional algorithm, run experiments on proper datasets, rewrite the introduction to make it clearer, correct English language errors, add another relevant paper to the literature review, or avoid writing papers altogether.
\begin{itemize}
    \item Specify \textit{exact} locations (e.g., "Section 3.2, Table 4")
    \item Provide implementable steps (e.g., "Add t-test results comparing X/Y in Table 3")
\end{itemize}


\section*{Final Decision Framework}
\textbf{Scale:} 1 (Poor) to 5 (Excellent)
\begin{itemize}
    \item \textcolor{rating5}{\textbf{5: Excellent}} -- Accept as-is, recommended to continue the work for future A*/Q1 publications
    \item \textcolor{rating4}{\textbf{4: Good}} -- Meets criteria well, recommended to continue the work for future A*/Q1 publications, however, major work is required
    \item \textcolor{rating3}{\textbf{3: Adequate}} -- Meets most criteria; needs moderate work for SSPP
    \item \textcolor{rating2}{\textbf{2: Weak}} -- Partially meets criteria; major revisions are required for SSPP
    \item \textcolor{rating1}{\textbf{1: Poor}} -- Fails criteria; unacceptable flaws
\end{itemize}


\section*{Review starts here:}
\section*{Core Criteria}
\begin{enumerate}
    \item \textbf{Preliminary Novel Work}
    \begin{itemize}
        \item[--] Explores new direction with concrete evidence?
        \item[--] Proof-of-concept validation beyond hypothetical?
        \item[--] Clear potential to inspire future work?
    \end{itemize}
    \textbf{Rating:} 5/5 \\
    Strengths: The approach is novel and interesting. 
The work proposes several methods for evaluating token homogenization, combined with the construction of a diagnostic dataset.\\
    Weaknesses: It is unclear whether the observed phenomena lead to degradation in model performance.
The paper does not investigate whether the proposed dataset modifications (e.g., shifting important information to the beginning or end) affect LLM performance on downstream tasks such as review sentiment classification. Consequently, the observed increase in homogenization on this data cannot be directly interpreted as having harmful effects. \\
    Recommendations: Investigate the impact of the proposed modifications on downstream task performance and address the above questions directly.
    
    \item \textbf{Application Analysis}
    \begin{itemize}
        \item[--] Evaluates strengths/weaknesses (metrics, tradeoffs)?
        \item[--] Provides actionable takeaways?
        \item[--] Sufficient documentation for \textit{reproducibility}?
    \end{itemize}
    \textbf{Rating:} 4/5 \\
    Strengths: The paper evaluates seven different metrics for measuring token homogenization under positional bias and compares results for natural and paraphrased datasets. \\
    Weaknesses: The description of paraphrased dataset creation is insufficient.
The selection process for dataset examples, the balance of classes (e.g., positive/negative reviews), and paraphrasing quality is not documented. \\
    Recommendations: Analyze differences between paraphrased and original data in terms of sentence length, fluency, and other shallow features.
Provide evidence that the paraphrasing is correct (e.g., via LLM-based quality judgments).
Include statistics on the position of important phrases, phrase lengths, and class distribution in the dataset.
    
    \item \textbf{Empirical Foundation}
    \begin{itemize}
        \item[--] \textit{Importance:} Provides value for future research?
        \item[--] \textit{Reliability:} Statistically sound methods?
        \item[--] \textit{Documentation:} Enables full replication?
    \end{itemize}
    \textbf{Rating:} 4/5 \\
    Strengths: The paper calculates multiple metrics related to embedding direction homogenization, resulting in a more comprehensive picture.
The results can provide valuable insights into general LLM properties, such as metric distributions across layers. \\
    Weaknesses: Only average values across data samples are reported, without any measure of variance. \\
    Recommendations: Include standard deviations (or other dispersion measures) for all reported parameters to better represent variability.
    
    \item \textbf{Methodological Quality}
    \begin{itemize}
        \item[--] \textit{Design:} Methods match goals?
        \item[--] \textit{Execution:} Replicable protocols?
        \item[--] \textit{Limitations:} Critical discussion of constraints?
    \end{itemize}
    \textbf{Rating:} 4/5 \\
    Strengths: The homogenization metrics are relevant.
Interesting hypotheses about token homogenization under positional bias are introduced. \\
    Weaknesses: Positional bias is defined as “systematic neglect of information in certain positions,” but the experiments remove information from those positions instead of testing whether the model neglects it.
Token homogenization is defined as “convergence of tokens toward uniformity across layers,” but the analysis interprets overall lower metric values for the transformed dataset across layers as evidence of homogenization, which does not strictly follow from the definition. \\
    Recommendations: Ensure that definitions, hypotheses, experimental design, and interpretations are fully aligned.
In the results analysis, explicitly address the research questions set in the introduction and use consistent terminology.
    
    \item \textbf{Analysis \& Insight Depth}
    \begin{itemize}
        \item[--] Examines challenges/tradeoffs?
        \item[--] Contextualizes in broader research?
        \item[--] Delivers implementable recommendations?
    \end{itemize}
    \textbf{Rating:} 4/5 \\
    Strengths: The literature review is solid and provides good context. \\
    Weaknesses: The analysis of LLM behavior across layers is limited. \\
    Recommendations: Provide a deeper analysis for and against the stated hypotheses, supported by the results.
For example, the anisotropy score behaves differently in LLaMA and Gemma: LLaMA shows near-complete isotropy in the highest layer, whereas Gemma maintains higher values. Discuss what these differences imply from the homogenization perspective.
    
    \item \textbf{Clarity \& Reproducibility}
    \begin{itemize}
        \item[--] Logical structure?
        \item[--] Code/data available?
        \item[--] Accessible to adjacent fields?
    \end{itemize}
    \textbf{Rating:} 4/5 \\
    Strengths: The paper introduces interesting mathematical ideas for different homogenization metrics. \\
    Weaknesses: Only part of the proposed theoretical framework is applied in the experiments. \\
    Recommendations: Establish a clearer connection between the formalization in Section~\ref{sec:positional_bias} and the metrics presented in Methodology.
\end{enumerate}

\\

\section*{Final Decision}
\textbf{Decision:} \textbf{4} (keep only one, remove others).
